Comparing Bad Apples to Good Oranges: Aligning Large Language Models via Joint Preference Optimization

A common technique for aligning large language models (LLMs) relies on acquiring human preferences by comparing multiple generations conditioned on a fixed context. This method, however, relies solely on pairwise comparisons, where the generations are evaluated within an identical context. While effective to such conditional preferences often fail to encompass the nuanced and multidimensional nature of human preferences. In this work, we revisit the traditional paradigm of preference acquisition and propose a new axis based on eliciting preferences jointly over the instruction-response pairs. Unlike prior preference optimizations, which are designed for conditional ranking protocols (e.g., DPO), we propose Joint Preference Optimization (JPO), a new preference optimization objective that upweights the joint probability of the chosen instruction-response pair over the rejected instruction-response pair. Interestingly, LLMs trained with joint instruction-response preference data using JPO outperform LLM trained with DPO by $5.2\%$ and $3.3\%$ win-rate for summarization and open-ended dialogue datasets, respectively. Our findings reveal that joint preferences over instruction and response pairs can significantly enhance the alignment of LLMs by tapping into a broader spectrum of human preference elicitation. The data and code is available at https://github.com/Hritikbansal/dove.

==> sections/short_relatedwork.tex <==
\section{Related Work}
\label{sec:relatedwork}


% \paragraph{Alignment using Reinforcement Learning.} Large Language Models (LLMs) showcase impressive few-shot performance \cite{brown2020language} which is further improved by instruction tuning followed by alignment with preferences data  \cite{victor2022multitask, ouyang2022training, dubois2023alpacafarm, zheng2023judging, schulman2017proximal, wang2023beyond}. This alignment is usually done by first optimizing for a reward model on a preference data \cite{bradley1952rank}, followed by aligning the LLMs distribution to maximize the learned reward model (using RLHF/RLAIF). In this work, we show that preference acquisition is a complex phenomenon and elicits joint preferences over instruction-response data. Further, we study the interactions between joint preferences and the traditional approach of conditional rankings for preference elicitation. 

% \paragraph{Reward Free Policy Alignment.} \cite{dpo} introduced Direct Preference Optimization (DPO) that mitigates the instability due to PPO for reward maximization by skipping reward modeling and optimizing directly within the model parameter space. \cite{pal2024smaug} adds an explicit penalty term to avoid a reduction in the likelihood of preferred pairs. \cite{ethayarajh2024kto} improves over DPO by using human-aware loss based on prospect theory.  Concurrent to our work, \cite{yin2024relative} explores the comparison between two responses for non-identical instructions. However, they do not uncover new preference acquisition paths, and instead rely on augmenting the existing conditional rankings. In addition, we introduce \name, a novel preference optimization, complementary to existing works, that learns from joint preferences over instruction-response data and achieves good performance on diverse tasks. We refer to \S \ref{sec:detailed_relatedwork} for a detailed related work.

\paragraph{Alignment using Reinforcement Learning.} Large Language Models (LLMs) showcase impressive zero-shot and few-shot performance \cite{brown2020language} with instruction tuning further improving their downstream performance \cite{victor2022multitask}. Not all responses for a prompt are preferable due to a variety of reasons, thus aligning them with human preference is now a common step in fine-tuning the pipeline. This alignment is usually done by first optimizing for a reward model on preference data \cite{bradley1952rank, likert1932technique, bansal2023peering}, followed by aligning the LLMs distribution that maximizes the learned reward model using Reinforcement Learning (RLHF) \cite{schulman2017proximal, ouyang2022training}, with optional Divergence penalty \cite{wang2023beyond} to avoid deviating from the reference policy. Despite the success of RLHF, collecting human feedback can be challenging, however, \cite{dubois2023alpacafarm, lu2024llmscore, zheng2023judging}  observe that LLMs can provide feedback 
motivating Reinforcement Learning through AI feedback (RLAIF). In this work, we show that preference acquisition is a complex phenomenon and elicit joint preferences over instruction-response data. Further, we study the interactions between joint preferences and traditional approach of conditional rankings for preference elicitation. 


\paragraph{Reward Free Policy Alignment.} \cite{dpo} introduced Direct Preference Optimization (DPO) that mitigates the instability due to PPO for reward maximization by optimizing directly within the model parameter space, hence by-passing the reward modeling step. \cite{liu2024lipo} extends this framework where instead of two responses, alignment is done over the list of responses while \cite{liu2023statistical} improves DPO using statistical rejection sampling. \cite{amini2024direct} provides an offset in the DPO objective to increase the margins and \cite{pal2024smaug} suggests adding an explicit penalty term to avoid a reduction in the likelihood of preferred pairs over the DPO training. Contrary to our work where compare the joint distributions, \cite{yin2024relative} proposes RPO that compares the conditional likelihood of a winning response with the losing response of another prompt. Beyond DPO, more recently \cite{ethayarajh2024kto} proposed a human-aware loss function-based framework using prospect theory named KTO, and \cite{azar2023general} proposes IPO that uses human preferences expressed as pairwise preferences. Lastly, \cite{zhao2022calibrating} uses sequence likelihood calibration to align the model from human preference. Here, we introduce \name, a novel preference optimization, complementary to existing works, that learns from joint preferences over instruction-response data and achieves good performance on diverse tasks.

